Towards Diverse and Faithful One-shot Adaption of Generative Adversarial Networks

One-shot generative domain adaption aims to transfer a pre-trained generator on one domain to a new domain using one reference image only. However, it remains very challenging for the adapted generator (i) to generate diverse images inherited from the pre-trained generator while (ii) faithfully acquiring the domain-specific attributes and styles of the reference image. In this paper, we present a novel one-shot generative domain adaption method, i.e., DiFa, for diverse generation and faithful adaptation. For global-level adaptation, we leverage the difference between the CLIP embedding of reference image and the mean embedding of source images to constrain the target generator. For local-level adaptation, we introduce an attentive style loss which aligns each intermediate token of adapted image with its corresponding token of the reference image. To facilitate diverse generation, selective cross-domain consistency is introduced to select and retain the domain-sharing attributes in the editing latent $\mathcal{W}+$ space to inherit the diversity of pre-trained generator. Extensive experiments show that our method outperforms the state-of-the-arts both quantitatively and qualitatively, especially for the cases of large domain gaps. Moreover, our DiFa can easily be extended to zero-shot generative domain adaption with appealing results. Code is available at https://github.com/1170300521/DiFa.

==> figText/mean_vs_corr.tex <==
\begin{figure}[h]
   \vspace{-1em}
  \begin{center}
  \includegraphics[width=.99\linewidth]{figures/mean_vs_corr.pdf}
  \end{center}
  \vspace{-2mm}
  \caption{
  \textbf{Qualitative comparisons between one-stage and two-stage methods using directional CLIP loss only}.
  The first and second columns show reference images in domain $B$ and their corresponding images in domain $A$ respectively.
  The first row shows source images in domain $A$.
  The main difference between one-stage and two-stage methods is the estimation of source domain embedding.
  The one-stage method use the mean embedding of sampled source images while the two-stage method use the embedding of the corresponding source image of the reference image.
  }
    \label{fig:mean_vs_corr}
  \vspace{-2.5mm}
\end{figure}
